Generative AI for Multiple Choice STEM Assessments

Artificial intelligence (AI) technology enables a range of enhancements in computer-aided instruction, from accelerating the creation of teaching materials to customizing learning paths based on learner outcomes. However, ensuring the mathematical accuracy and semantic integrity of generative AI output remains a significant challenge, particularly in Science, Technology, Engineering and Mathematics (STEM) disciplines. In this study, we explore the use of generative AI in which "hallucinations", typically viewed as undesirable inaccuracies, can instead serve a pedagogical purpose. Specifically, we investigate the generation of plausible but incorrect alternatives for multiple choice assessments, where credible distractors are essential for effective assessment design. We describe the Moebius platform for online instruction, with particular focus on its architecture for handling mathematical elements through specialized semantic packages that support dynamic, parameterized STEM content. We examine methods for crafting prompts that interact effectively with these mathematical semantics to guide the AI in generating high-quality multiple choice distractors. Finally, we demonstrate how this approach reduces the time and effort associated with creating robust teaching materials while maintaining academic rigor and assessment validity.

==> IfExistsUseBBL.tex <==
% If this file exists, then the .bbl file is used instead of calling bibtex.
% It cannot be empty.   To force bibtex to run, rename this file to something else.
